Random Features for Compositional Kernels

We describe and analyze a simple random feature scheme (RFS) from prescribed compositional kernels. The compositional kernels we use are inspired by the structure of convolutional neural networks and kernels. The resulting scheme yields sparse and efficiently computable features. Each random feature can be represented as an algebraic expression over a small number of (random) paths in a composition tree. Thus, compositional random features can be stored compactly. The discrete nature of the generation process enables de-duplication of repeated features, further compacting the representation and increasing the diversity of the embeddings. Our approach complements and can be combined with previous random feature schemes.

==> abs.tex <==
 We describe and analyze a simple random feature scheme (RFS) from prescribed
 compositional kernels. The compositional kernels we use are inspired by the
 structure of convolutional neural networks and kernels. The resulting scheme
 is simple and yields sparse and efficiently computable features. Each random
 feature can be represented as an algebraic expression over a {\em small}
 number of (random) paths in a composition tree. Thus, compositional random
 features can be stored very compactly. The discrete nature of the generation
 process enables de-duplication of repeated features, further compacting the
 representation and increasing the diversity of the embeddings. Our approach
 rather complements and can be combined with previous random feature schemes.

